Memory-Efficient Gradient Unrolling for Large-Scale Bi-level Optimization

Bi-level optimization (BO) has become a fundamental mathematical framework for addressing hierarchical machine learning problems. As deep learning models continue to grow in size, the demand for scalable bi-level optimization solutions has become increasingly critical. Traditional gradient-based bi-level optimization algorithms, due to their inherent characteristics, are ill-suited to meet the demands of large-scale applications. In this paper, we introduce $\textbf{F}$orward $\textbf{G}$radient $\textbf{U}$nrolling with $\textbf{F}$orward $\textbf{F}$radient, abbreviated as $(\textbf{FG})^2\textbf{U}$, which achieves an unbiased stochastic approximation of the meta gradient for bi-level optimization. $(\text{FG})^2\text{U}$ circumvents the memory and approximation issues associated with classical bi-level optimization approaches, and delivers significantly more accurate gradient estimates than existing large-scale bi-level optimization approaches. Additionally, $(\text{FG})^2\text{U}$ is inherently designed to support parallel computing, enabling it to effectively leverage large-scale distributed computing systems to achieve significant computational efficiency. In practice, $(\text{FG})^2\text{U}$ and other methods can be strategically placed at different stages of the training process to achieve a more cost-effective two-phase paradigm. Further, $(\text{FG})^2\text{U}$ is easy to implement within popular deep learning frameworks, and can be conveniently adapted to address more challenging zeroth-order bi-level optimization scenarios. We provide a thorough convergence analysis and a comprehensive practical discussion for $(\text{FG})^2\text{U}$, complemented by extensive empirical evaluations, showcasing its superior performance in diverse large-scale bi-level optimization tasks. Code is available at https://github.com/ShenQianli/FG2U.

==> tex/0-abstract_no_cmd.tex <==
Bi-level optimization (BO) has become a fundamental mathematical framework for addressing hierarchical machine learning problems.
As deep learning models continue to grow in size, the demand for scalable BO solutions has become increasingly critical.
Traditional gradient-based bi-level optimization algorithms, due to their inherent characteristics, are ill-suited to meet the demands of large-scale applications.
In this paper, we introduce **F**orward **G**radient **U**nrolling with **F**orward **G**radient, abbreviated as **$($FG$)^2$U**, which achieves an unbiased stochastic approximation of the meta gradient for bi-level optimization.
$($FG$)^2$U circumvents the memory and approximation issues associated with classical bi-level optimization approaches, and delivers significantly more accurate gradient estimates than existing large-scale bi-level optimization approaches.
Additionally, $($FG$)^2$U is inherently designed to support parallel computing, enabling it to effectively leverage large-scale distributed computing systems to achieve significant computational efficiency.
In practice, $($FG$)^2$U and other methods can be strategically placed at different stages of the training process to achieve a more cost-effective two-phase paradigm.
Further, $($FG$)^2$U is easy to implement within popular deep learning frameworks, and can be conveniently adapted to address more challenging zeroth-order bi-level optimization scenarios.
We provide a thorough convergence analysis and a comprehensive practical discussion for $($FG$)^2$U, complemented by extensive empirical evaluations, showcasing its superior performance in diverse large-scale bi-level optimization tasks.

==> tex/2-2-2-if.tex <==
\subsubsection{Implicit Function}\label{sec:if}

Another idea for computing the implicit gradient is to utilize the implicit function theorem (IFT)~\cite{ift}.
Suppose that the inner optimality $\nabla_\btheta g(\btheta_T(\bphi), \bphi) \approx 0$ is approximately achieved by sufficient inner optimization steps.
If $g$ is second-order differentiable, by applying the implicit function theorem and taking the first-order derivative of $\bphi$, 

\begin{equation}\label{eq:ift}
\begin{aligned}
    \frac{\partial^2 g(\btheta_T(\bphi), \bphi)}{\partial \btheta_T^2} \frac{d\btheta_T(\bphi)}{d\bphi}+ \frac{\partial^2 g(\btheta_T(\bphi), \bphi)}{\partial \btheta_T \partial \bphi} \approx 0.
\end{aligned}
\end{equation}

Then, if the Hessian is further assumed to be invertible, the meta gradient can be approximated as


\begin{equation}\label{eq:if}
    \nabla_\bphi h(\bphi) \approx -\frac{\partial f(\btheta_T(\bphi), \bphi)}{\partial \btheta_T} \left(\frac{\partial^2 g(\btheta_T(\bphi), \bphi)}{\partial \btheta_T^2}\right)^{-1} \frac{\partial^2 g(\btheta_T(\bphi), \bphi)}{\partial \btheta_T \partial \bphi} + \frac{\partial f(\btheta_T(\bphi), \bphi)}{\partial \bphi}.
\end{equation}

The main challenge lies in the computation of the inverse Hessian matrix, which is intractable when $\btheta$ is of high dimensionality.
Fortunately, several iterative inverse Hessian vector product (\texttt{ihvp}) approximators requiring only Hessian vector product (\texttt{hvp}) and $\mathcal{O}(M)$ space are well studied in the literature, based on Conjugate Gradient~\cite{cg, imaml_cg}, Neumann Series~\cite{neumann_1, two_timescale, stocbio} and low-rank approximation~\cite{singh2020woodfisher, hataya2023nystrom}.

\textbf{Weakness (IF): Approximation Errors}. \
The errors of IF emanate from two distinct sources
Firstly, IFT presupposes that the Karush-Kuhn-Tucker (KKT) conditions of the inner problem are satisfied, leading to an approximation error in~\eqref{eq:ift} when iterative approximations of the inner solutions are used.
Secondly, the singular nature of the Hessian within neural network training~\cite{singular} leads to costly and unstable inverse Hessian approximation in practical applications, with a heavy reliance on engineering efforts~\cite{choe2024sama}.
% These errors are particularly burdensome to control, especially given that they cannot be effectively mitigated through distributed computing.

To reduce the computational cost,
Hessian-free approaches~\cite{hessian_free_1, hessian_free_2, choe2024sama} propose approximating the Hessian as an identity matrix, incorporating additional assumptions about the inner model and objective. 
However, these numerous assumptions often diverge from practical scenarios, resulting in significant approximation errors and consequently inducing suboptimal outcomes.
See~\cref{appendix:if_bias} for a more detailed discussion and empirical evidence.

==> tex/2-2-3-vf.tex <==
\subsubsection{Value Function (VF)}

The VF-based methodology~\cite{vf1, vf2_bome, vf3, vf4_f2sa} considers an equivalent reformulation of the original optimization problem as outlined in~\eqref{eq:T-step_objective}:

\begin{equation}\label{eq:vf}
\begin{aligned}
\mathop{\min}_{\btheta, \bphi}\ f(\btheta, \bphi) \quad s.t.\ g(\btheta, \bphi) \le g(\btheta_T(\bphi), \bphi).
\end{aligned}
\end{equation}

This reformulation casts the standard bilevel optimization (BO) challenge into a constrained single-level optimization framework. 
VF-based methods circumvent the need for second-order computations and have demonstrated near-optimal complexity, comparable to second-order methodologies in deterministic settings, as reported in~\cite{f2sa_theory}.

\textbf{Weakness (VF): stochastic optimization}. \ 
VF-based strategies have yet to gain widespread acceptance in practical ML applications. 
This limited adoption is primarily attributed to the challenges these methods face in addressing large-scale stochastic problems, where the complexity significantly impedes their performance~\cite{zhang2023introduction}.


==> tex/3-X-variance_reduction.tex <==
\subsection{Variance Reduction}

\begin{equation}
    \begin{aligned}
        \mathop{\min}_{\mathbf{\phi}}\  h(\phi):=f&(\hat{\mathbf{\theta}}^*(\mathbf{\phi}), \mathbf{\phi})
        \quad s.t. \quad \hat{\mathbf{\theta}}^*(\mathbf{\phi}) = \mathbf{\theta}_T(\mathbf{\phi}),\\  
        where \quad \theta_0 = \Omega_0(\phi), &\quad \mathbf{\theta}_t(\mathbf{\phi}) = \Omega_t(\mathbf{\theta}_{t-1}, \mathbf{\phi}),\ \  t = 1,\dots,T
    \end{aligned}
\end{equation}

The gradient

\begin{equation}
    {\nabla} h(\phi) := \frac{\partial f}{\partial \mathbf{\phi}} + \frac{\partial f}{\partial \mathbf{\theta}_T} \frac{d\mathbf{\theta}_T}{d\mathbf{\phi}}
\end{equation}

Following the chain rule, a recuisive formulas for computing $\frac{d\mathbf{\theta}_T(\mathbf{\phi})}{d\mathbf{\phi}}$ can be derived as
\begin{equation}
    \underbrace{\frac{d \mathbf{\theta}_t}{d\mathbf{\phi}}}_{Z_t} = \underbrace{\frac{\partial \Omega_t(\mathbf{\theta}_{t-1}, \mathbf{\phi})}{\partial \mathbf{\theta}_{t-1}}}_{A_t} \underbrace{\frac{d \mathbf{\theta}_{t-1}}{d\mathbf{\phi}}}_{Z_{t-1}} + \underbrace{\frac{\partial \Omega_t(\mathbf{\theta}_{t-1}, \mathbf{\phi})}{\partial \mathbf{\phi}}}_{B_t}, \  t=1,\dots,T,
    \label{eq:fmd}
\end{equation}

which leads to

\begin{equation}
     Z_T = \sum_{i=0}^T A_T\cdots A_{i+1}B_i
\end{equation}

A biased estimation with the first $K < T$ steps truncated

\begin{equation}
    \tilde{Z}_T = \sum_{i=K}^T A_T\cdots A_{i+1}B_i = Z_T - \sum_{i=0}^{K-1} A_T\cdots A_{i+1}B_i
\end{equation}

The corresponding truncated gradient 

\begin{equation}
   \tilde{\nabla} h(\phi) := \frac{\partial f}{\partial \mathbf{\phi}} + \frac{\partial f}{\partial \mathbf{\theta}_{T}} \tilde{Z}_T = {\nabla} h(\phi) - \frac{\partial f}{\partial \mathbf{\theta}_{T}} \sum_{i=0}^{K-1} A_T\cdots A_{i+1}B_i
\end{equation}

Let $\mathbf{v}_{1:b}$ denote $b$ \emph{i.i.d.} random directions sampled from $p(\cdot)$.
The forward gradient $\hat{\nabla} h_i$ and the truncated forward gradient $\tilde{{\nabla} h}_i$ along the direction $\mathbf{v}_i$, where $i \in \{1,\dots,b\}$, will be repe

\begin{equation}
    \hat{\nabla} h_i(\phi) = {\nabla} h(\phi) \mathbf{v}_i\mathbf{v}_i^T, \quad\tilde{\nabla} h_i(\phi) = \tilde{\nabla} h(\phi) \mathbf{v}_i\mathbf{v}_i^T
\end{equation}

The variance reduction version

\begin{equation}
    \hat{\nabla} h_i^{\text{VR}}(\phi) = \hat{\nabla} h_i(\phi) - [\hat{\nabla} h_i(\tilde{\phi}) - \frac{1}{b}\sum_{j=1}^b \hat{\nabla} h_j(\tilde{\phi})],
\end{equation}

The variance reduction version with truncated baseline term

\begin{equation}
   \tilde{\nabla} h_i^{\text{VR}}(\phi) = \hat{\nabla} h_i(\phi) - [\tilde{{\nabla} h}_i(\tilde{\phi}) - \frac{1}{b}\sum_{j=1}^b\tilde{\nabla} h_j(\tilde{\phi})],
\end{equation}



% \begin{algorithm}[t]
% \caption{$\mathbf{\textbf{T(FG)}^2}$\textbf{U}: Truncated Forward Gradient Unrolling with Forward Gradient}\label{alg:TFG2}
% \begin{algorithmic}[1]
% \REQUIRE Initial inner parameters $\theta_0$, initial meta parameter $\phi_0$, total meta steps $S$, meta update mappings $\Psi_{1:S}$, truncated steps $K$, checkpoint update interval $L$
% \FOR{$s = 1,\dots,S$}
%     \IF{$s \text{ mode } L = 1$}
%     \STATE $\tilde{\theta}_0 \leftarrow \theta_0$
%     \FOR{$t=1,\dots,T-K$}
%         \STATE $\tilde{\theta}_t \leftarrow \Omega_t(\tilde{\theta}_{t-1}, \phi_{s-1})$
%     \ENDFOR
%     \ENDIF
%     \FOR{$i=1,\dots,b$}
%         \STATE $\tilde{\mathbf{c}}_{T-K, i} \leftarrow \mathbf{0}$
%         \STATE Sample $\mathbf{v}_i \sim \textbf{p}(\cdot)$
%         \FOR{$t=T-K+1,\dots,T$}
%             \STATE $\tilde{\theta}_t \leftarrow \Omega_t(\tilde{\theta}_{t-1}, \phi_{s-1})$
%             \STATE $\tilde{\mathbf{c}}_{t, i} \leftarrow \frac{\partial \Omega_t(\tilde{\theta}_{t-1}, \phi_{s-1})}{\partial \tilde{\theta}_{t-1}} \tilde{\mathbf{c}}_{t, i} + \frac{\partial \Omega_t(\tilde{\theta}_{t-1}, \phi_{s-1})}{\partial \phi_{s-1}}\mathbf{v}_i$
%         \ENDFOR
%         \STATE $\tilde{w}_i \leftarrow \frac{\partial f(\tilde{\theta}_t, \phi_{s-1})}{\partial \tilde{\theta}_t} \tilde{\mathbf{c}}_{T, i} + \frac{\partial f(\tilde{\theta}_t, \phi_{s-1})}{\partial \phi_{s-1}}\mathbf{v}_i$
%     \ENDFOR
%     \STATE $\hat{\nabla} h(\phi_{s-1}) = \frac{1}{b} \sum_{i=1}^b \tilde{w}_i \mathbf{v}_i^T$
%     \STATE $\phi_s \leftarrow \Psi_s(\phi_{s-1}, \hat{\nabla} h(\phi_{s-1}))$
% \ENDFOR
% \RETURN $\phi_S$
% \end{algorithmic}
% \end{algorithm}


==> tex/4.4-wrench.tex <==
% \begin{table}
%     \centering
%     \begin{tabular}{ccccccc}
%         & TREC  & SemEval & IMDB & ChemProt & AGNews & Yelp \\
%         \hline
%         gold (impl.) & 96.27\small{(0.83)} & 91.67\small{(0.50)} & 87.49\small{(0.46)} & 76.54\small{(0.06)} & 93.17\small{(0.17)} & 94.27\small{(0.35)}\\
%         \hline
%         finetune~\cite{zhang2021wrench} & 66.56\small{(2.31)} & 83.93\small{(1.74)} & 79.73\small{(2.60)} & 56.09\small{(1.08)} & 86.27\small{(0.53)} & 82.26\small{(3.50)} \\
%         finetune~\cite{choe2024sama} & 67.93\small{(2.55)} & 79.28\small{(1.78)} & 78.16\small{(2.28)} & 57.35\small{(1.43)} & 85.79\small{(0.49)} & 84.32\small{(2.55)}\\
%         \hline
%         finetune-MV (impl.) & 65.93\small{(0.13)} & 79.61\small{(2.98)} & 76.12\small{(0.58)} & 51.73\small{(1.66)} & 87.23\small{(0.57)} & 75.10\small{(1.79)}\\
%         finetune-SL (impl.) & 68.13\small{(0.16)} & 78.61\small{(0.98)} & 76.35\small{(0.64)} & 55.26\small{(1.81)} & 86.84\small{(0.13)} & 75.85\small{(1.33)}\\
%         \hline
%         COSINE~\cite{yu2020cosine}& 76.56\small{(0.08)} & 86.80\small{(0.46)} & 82.98\small{(0.05)} & 58.47\small{(0.08)} & 87.03\small{(0.00)} & 89.22\small{(0.05)}\\
%         SAMA-R~\cite{choe2024sama}& 85.73\small{(0.81)} & 89.67\small{(0.67)} & 84.31\small{(1.86)} & 76.89\small{(1.39)} & 89.05\small{(0.34)} & 93.64\small{(0.40)}\\
%         SAMA-R\&C~\cite{choe2024sama} & 87.93\small{(1.17)} & 88.83\small{(2.32)} & 85.71\small{(0.82)} & 77.78\small{(0.59)} & 89.79\small{(0.27)} & 93.77\small{(0.08)}\\
%         \hline
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:wrench}
% \end{table}

